The Machado--Bishop theorem in the uniform topology

The Machado--Bishop theorem for weighted vector-valued functions vanishing at infinity has been extensively studied. In this paper, we give an analogue of Machado's distance formula for bounded weighted vector-valued functions. A number of applications are given; in particular, some types of the Bishop--Stone--Weierstrass theorem for bounded vector-valued continuous spaces in the uniform topology are discussed; the splitting of $C(I \times J, X \otimes Y)$ as the closure of $C(I, X) \otimes C(J, Y)$ in different senses and the extension of continuous vector-valued functions are studied.

==> ThmAndAutoref.tex <==
\RequirePackage{amsthm, aliascnt}

\theoremstyle{theorem}
\newtheorem{thm}{Theorem}[section]

\newtheorem*{thm*}{Theorem}

\newaliascnt{corollary}{thm}
\newtheorem{cor}[corollary]{Corollary}
\aliascntresetthe{corollary}

\newaliascnt{lemma}{thm}
\newtheorem{lem}[lemma]{Lemma}
\aliascntresetthe{lemma}

\newaliascnt{sublemma}{thm}
\newtheorem{slem}[sublemma]{Sublemma}
\aliascntresetthe{sublemma}

\theoremstyle{definition}
\newaliascnt{definition}{thm}
\newtheorem{defi}[definition]{Definition}
\aliascntresetthe{definition}

\newaliascnt{example}{thm}
\newtheorem{exa}[example]{Example}
\aliascntresetthe{example}

%\theoremstyle{Remark}
\newaliascnt{remark}{thm}
\newtheorem{rmk}[remark]{Remark}
\aliascntresetthe{remark}

\newcommand{\thmautorefname}{Theorem}
\newcommand{\corollaryautorefname}{Corollary}
\newcommand{\lemmaautorefname}{Lemma}
\newcommand{\definitionautorefname}{Definition}
\newcommand{\remarkautorefname}{Remark}
\newcommand{\sublemmaautorefname}{Sublemma}%
\newcommand{\exampleautorefname}{Example}


\renewcommand{\chapterautorefname}{Chapter}
\renewcommand{\sectionautorefname}{Section}
\renewcommand{\subsubsectionautorefname}{Section}
\renewcommand{\subsectionautorefname}{Section}

%\def\figureautorefname{Figure}

\theoremstyle{theorem}
\newtheorem{thmA}{Theorem}
\renewcommand{\thethmA}{\Alph{thmA}}

\newcommand{\thmAautorefname}{Theorem}

\theoremstyle{theorem}
\newtheorem{thmI}{Theorem}
\renewcommand{\thethmI}{\Roman{thmI}}

\newaliascnt{corI}{thmI}
\newtheorem{corI}[corI]{Corollary}
\aliascntresetthe{corI}

\newcommand{\thmIautorefname}{Theorem}
\newcommand{\corIautorefname}{Corollary}

% begin appendix autoref patch [\autoref subsections in appendix](https://tex.stackexchange.com/questions/149807/autoref-subsections-in-appendix)
\RequirePackage{etoolbox}
\makeatletter
\patchcmd{\hyper@makecurrent}{%
	\ifx\Hy@param\Hy@chapterstring
	\let\Hy@param\Hy@chapapp
	\fi
}{%
	\iftoggle{inappendix}{%
		\@checkappendixparam{chapter}%
		\@checkappendixparam{section}%
		\@checkappendixparam{subsection}%
		\@checkappendixparam{subsubsection}%
		\@checkappendixparam{paragraph}%
		\@checkappendixparam{subparagraph}%
	}{}%
}{}{\errmessage{failed to patch}}

\newcommand*{\@checkappendixparam}[1]{%
	\def\@checkappendixparamtmp{#1}%
	\ifx\Hy@param\@checkappendixparamtmp
	\let\Hy@param\Hy@appendixstring
	\fi
}

\newtoggle{inappendix}
\togglefalse{inappendix}
\apptocmd{\appendix}{\toggletrue{inappendix}}{}{\errmessage{failed to patch}}
\@ifpackageloaded{appendix}
{
	\apptocmd{\appendices}{\toggletrue{inappendix}}{}{\errmessage{failed to patch}}
	\apptocmd{\subappendices}{\toggletrue{inappendix}}{}{\errmessage{failed to patch}}
}
{}
\makeatother

